Can Taxonomy Help? Improving Semantic Question Matching using Question Taxonomy

In this paper, we propose a hybrid technique for semantic question matching. It uses our proposed two-layered taxonomy for English questions by augmenting state-of-the-art deep learning models with question classes obtained from a deep learning based question classifier. Experiments performed on three open-domain datasets demonstrate the effectiveness of our proposed approach. We achieve state-of-the-art results on partial ordering question ranking (POQR) benchmark dataset. Our empirical analysis shows that coupling standard distributional features (provided by the question encoder) with knowledge from taxonomy is more effective than either deep learning (DL) or taxonomy-based knowledge alone.

==> COLING Camera Ready (By IITP)/refs.tex <==
\begin{thebibliography}{}

\bibitem[\protect\citename{Bahdanau \bgroup et al.\egroup
  }2014]{bahdanau2014neural}
Dzmitry Bahdanau, Kyunghyun Cho, and Yoshua Bengio.
\newblock 2014.
\newblock Neural machine translation by jointly learning to align and
  translate.
\newblock {\em arXiv preprint arXiv:1409.0473}.

\bibitem[\protect\citename{Bian \bgroup et al.\egroup }2008]{bian2008finding}
Jiang Bian, Yandong Liu, Eugene Agichtein, and Hongyuan Zha.
\newblock 2008.
\newblock Finding the right facts in the crowd: factoid question answering over
  social media.
\newblock In {\em Proceedings of the 17th international conference on World
  Wide Web}, pages 467--476. ACM.

\bibitem[\protect\citename{Bunescu and Huang}2010a]{bunescu2010learning}
Razvan Bunescu and Yunfeng Huang.
\newblock 2010a.
\newblock Learning the relative usefulness of questions in community qa.
\newblock In {\em Proceedings of the 2010 Conference on Empirical Methods in
  Natural Language Processing}, pages 97--107. Association for Computational
  Linguistics.

\bibitem[\protect\citename{Bunescu and Huang}2010b]{bunescu2010}
Razvan Bunescu and Yunfeng Huang.
\newblock 2010b.
\newblock Towards a general model of answer typing: Question focus
  identification.
\newblock In {\em Proceedings of The 11th International Conference on
  Intelligent Text Processing and Computational Linguistics (CICLing 2010), RCS
  Volume}, pages 231--242.

\bibitem[\protect\citename{Burke \bgroup et al.\egroup
  }1997]{burke1997question}
Robin~D Burke, Kristian~J Hammond, Vladimir Kulyukin, Steven~L Lytinen, Noriko
  Tomuro, and Scott Schoenberg.
\newblock 1997.
\newblock Question answering from frequently asked question files: Experiences
  with the faq finder system.
\newblock {\em AI magazine}, 18(2):57.

\bibitem[\protect\citename{Chang and Lin}2011]{chang2011libsvm}
Chih-Chung Chang and Chih-Jen Lin.
\newblock 2011.
\newblock Libsvm: a library for support vector machines.
\newblock {\em ACM Transactions on Intelligent Systems and Technology (TIST)},
  2(3):27.

\bibitem[\protect\citename{Cho \bgroup et al.\egroup }2014]{cho2014properties}
Kyunghyun Cho, Bart Van~Merri{\"e}nboer, Dzmitry Bahdanau, and Yoshua Bengio.
\newblock 2014.
\newblock On the properties of neural machine translation: Encoder-decoder
  approaches.
\newblock {\em arXiv preprint arXiv:1409.1259}.

\bibitem[\protect\citename{Chopra \bgroup et al.\egroup
  }2016]{chopra2016abstractive}
Sumit Chopra, Michael Auli, and Alexander~M Rush.
\newblock 2016.
\newblock Abstractive sentence summarization with attentive recurrent neural
  networks.
\newblock In {\em Proceedings of the 2016 Conference of the North American
  Chapter of the Association for Computational Linguistics: Human Language
  Technologies}, pages 93--98.

\bibitem[\protect\citename{Chung \bgroup et al.\egroup
  }2014]{chung2014empirical}
Junyoung Chung, Caglar Gulcehre, KyungHyun Cho, and Yoshua Bengio.
\newblock 2014.
\newblock Empirical evaluation of gated recurrent neural networks on sequence
  modeling.
\newblock {\em arXiv preprint arXiv:1412.3555}.

\bibitem[\protect\citename{Croce \bgroup et al.\egroup
  }2011]{Croce2011StructuredLS}
Danilo Croce, Alessandro Moschitti, and Roberto Basili.
\newblock 2011.
\newblock Structured lexical similarity via convolution kernels on dependency
  trees.
\newblock In {\em EMNLP}.

\bibitem[\protect\citename{Croce \bgroup et al.\egroup }2017]{Croce2017DeepLI}
Danilo Croce, Simone Filice, Giuseppe Castellucci, and Roberto Basili.
\newblock 2017.
\newblock Deep learning in semantic kernel spaces.
\newblock In {\em ACL}.

\bibitem[\protect\citename{Feng \bgroup et al.\egroup }2015]{feng2015applying}
Minwei Feng, Bing Xiang, Michael~R Glass, Lidan Wang, and Bowen Zhou.
\newblock 2015.
\newblock Applying deep learning to answer selection: A study and an open task.
\newblock In {\em 2015 IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 813--820. IEEE.

\bibitem[\protect\citename{Filice \bgroup et al.\egroup
  }2016]{Filice2016KeLPAS}
Simone Filice, Danilo Croce, Alessandro Moschitti, and Roberto Basili.
\newblock 2016.
\newblock Kelp at semeval-2016 task 3: Learning semantic relations between
  questions and answers.
\newblock In {\em SemEval@NAACL-HLT}.

\bibitem[\protect\citename{Gruber}1995]{gruber1995}
Thomas~R. Gruber.
\newblock 1995.
\newblock Toward principles for the design of ontologies used for knowledge
  sharing.
\newblock {\em Technical Report KSL 93-04}.

\bibitem[\protect\citename{Hinton \bgroup et al.\egroup
  }2012]{hinton2012improving}
Geoffrey~E Hinton, Nitish Srivastava, Alex Krizhevsky, Ilya Sutskever, and
  Ruslan~R Salakhutdinov.
\newblock 2012.
\newblock Improving neural networks by preventing co-adaptation of feature
  detectors.
\newblock {\em arXiv preprint arXiv:1207.0580}.

\bibitem[\protect\citename{Hovy \bgroup et al.\egroup }2001]{hovy2001toward}
Eduard Hovy, Laurie Gerber, Ulf Hermjakob, Chin-Yew Lin, and Deepak
  Ravichandran.
\newblock 2001.
\newblock Toward semantics-based answer pinpointing.
\newblock In {\em Proceedings of the first international conference on Human
  language technology research}, pages 1--7. Association for Computational
  Linguistics.

\bibitem[\protect\citename{Iyyer \bgroup et al.\egroup }2014]{iyyer2014neural}
Mohit Iyyer, Jordan Boyd-Graber, Leonardo Claudino, Richard Socher, and Hal
  Daum\'{e}~III.
\newblock 2014.
\newblock A neural network for factoid question answering over paragraphs.
\newblock In {\em Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, pages 633--644, Doha, Qatar, October.
  Association for Computational Linguistics.

\bibitem[\protect\citename{Jeon \bgroup et al.\egroup }2005]{jeon2005finding}
Jiwoon Jeon, W~Bruce Croft, and Joon~Ho Lee.
\newblock 2005.
\newblock Finding similar questions in large question and answer archives.
\newblock In {\em Proceedings of the 14th ACM international conference on
  Information and knowledge management}, pages 84--90. ACM.

\bibitem[\protect\citename{Kim}2014]{kimCNN}
Yoon Kim.
\newblock 2014.
\newblock Convolutional neural networks for sentence classification.
\newblock In {\em Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, pages 1746--1751. Association for
  Computational Linguistics.

\bibitem[\protect\citename{Kingma and Ba}2014]{kingma2014adam}
Diederik Kingma and Jimmy Ba.
\newblock 2014.
\newblock Adam: A method for stochastic optimization.
\newblock {\em arXiv preprint arXiv:1412.6980}.

\bibitem[\protect\citename{Lei \bgroup et al.\egroup
  }2016]{lei-EtAl:2016:N16-1}
Tao Lei, Hrishikesh Joshi, Regina Barzilay, Tommi Jaakkola, Kateryna
  Tymoshenko, Alessandro Moschitti, and Llu\'{i}s M\`{a}rquez.
\newblock 2016.
\newblock Semi-supervised question retrieval with gated convolutions.
\newblock In {\em Proceedings of the 2016 Conference of the North American
  Chapter of the Association for Computational Linguistics: Human Language
  Technologies}, pages 1279--1289, San Diego, California, June. Association for
  Computational Linguistics.

\bibitem[\protect\citename{Li and Manandhar}2011]{li2011improving}
Shuguang Li and Suresh Manandhar.
\newblock 2011.
\newblock Improving question recommendation by exploiting information need.
\newblock In {\em Proceedings of the 49th Annual Meeting of the Association for
  Computational Linguistics: Human Language Technologies-Volume 1}, pages
  1425--1434. Association for Computational Linguistics.

\bibitem[\protect\citename{Li and Roth}2002]{liroth2002}
Xin Li and Dan Roth.
\newblock 2002.
\newblock Learning question classifiers.
\newblock In {\em Proceedings of the 19th international conference on
  Computational linguistics, COLING 2002}, pages 1--7. Association for
  Computational Linguistics.

\bibitem[\protect\citename{M{\`a}rquez \bgroup et al.\egroup
  }2015]{marquez2015semeval}
Llu{\'\i}s M{\`a}rquez, James Glass, Walid Magdy, Alessandro Moschitti, Preslav
  Nakov, and Bilal Randeree.
\newblock 2015.
\newblock Semeval-2015 task 3: Answer selection in community question
  answering.
\newblock In {\em Proceedings of the 9th International Workshop on Semantic
  Evaluation (SemEval 2015)}.

\bibitem[\protect\citename{Mikolov \bgroup et al.\egroup
  }2013]{mikolov2013efficient}
Tomas Mikolov, Kai Chen, Greg Corrado, and Jeffrey Dean.
\newblock 2013.
\newblock Efficient estimation of word representations in vector space.
\newblock {\em arXiv preprint arXiv:1301.3781}.

\bibitem[\protect\citename{Mlynarczyk and
  Lytinen}2005]{mlynarczyk2005faqfinder}
S~Mlynarczyk and S~Lytinen.
\newblock 2005.
\newblock Faqfinder question answering improvements using question/answer
  matching.
\newblock {\em Proceedings of L\&T-2005-Human Language Technologies as a
  Challenge for Computer Science and Linguistics}.

\bibitem[\protect\citename{Moldovan \bgroup et al.\egroup }2000]{moldovan2000}
D~Moldovan, S~Harabagiu, M~Pasca, R~Mihalcea, R~Goodrum, R~Girji, and V~Rus.
\newblock 2000.
\newblock Lasso: A tool for surfing the answer net.
\newblock In {\em Proceedings 8th Text Retrieval Conference (TREC-8)}.

\bibitem[\protect\citename{Nakov \bgroup et al.\egroup }2016]{nakov16lluis}
Preslav Nakov, Llu{\i}s Marquez, Alessandro Moschitti, Walid Magdy, Hamdy
  Mubarak, Abed~Alhakim Freihat, Jim Glass, and Bilal Randeree.
\newblock 2016.
\newblock Semeval-2016 task 3: Community question answering.
\newblock In {\em Proceedings of the 10th International Workshop on Semantic
  Evaluation, SemEval}, volume~16.

\bibitem[\protect\citename{Ng and Kan}2015]{ng2015qanus}
Jun-Ping Ng and Min-Yen Kan.
\newblock 2015.
\newblock Qanus: An open-source question-answering platform.
\newblock {\em arXiv preprint arXiv:1501.00311}.

\bibitem[\protect\citename{Pennington \bgroup et al.\egroup
  }2014]{pennington2014glove}
Jeffrey Pennington, Richard Socher, and Christopher Manning.
\newblock 2014.
\newblock Glove: Global vectors for word representation.
\newblock In {\em Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, pages 1532--1543, Doha, Qatar, October.
  Association for Computational Linguistics.

\bibitem[\protect\citename{Rajpurkar \bgroup et al.\egroup }2016]{squad2016}
Pranav Rajpurkar, Jian Zhang, Konstantin Lopyrev, and Percy Liang.
\newblock 2016.
\newblock Squad: 100, 000+ questions for machine comprehension of text.
\newblock {\em CoRR}, abs/1606.05250.

\bibitem[\protect\citename{Severyn and Moschitti}2015]{severyn2015learning}
Aliaksei Severyn and Alessandro Moschitti.
\newblock 2015.
\newblock Learning to rank short text pairs with convolutional deep neural
  networks.
\newblock In {\em Proceedings of the 38th International ACM SIGIR Conference on
  Research and Development in Information Retrieval}, pages 373--382. ACM.

\bibitem[\protect\citename{Wang and Nyberg}2015]{wang-nyberg:2015:ACL-IJCNLP}
Di~Wang and Eric Nyberg.
\newblock 2015.
\newblock A long short-term memory model for answer sentence selection in
  question answering.
\newblock In {\em Proceedings of the 53rd Annual Meeting of the Association for
  Computational Linguistics and the 7th International Joint Conference on
  Natural Language Processing (Volume 2: Short Papers)}, pages 707--712,
  Beijing, China, July. Association for Computational Linguistics.

\bibitem[\protect\citename{Wang \bgroup et al.\egroup }2009]{wang2009syntactic}
Kai Wang, Zhaoyan Ming, and Tat-Seng Chua.
\newblock 2009.
\newblock A syntactic tree matching approach to finding similar questions in
  community-based qa services.
\newblock In {\em Proceedings of the 32nd international ACM SIGIR conference on
  Research and development in information retrieval}, pages 187--194. ACM.

\bibitem[\protect\citename{Zhang \bgroup et al.\egroup
  }2017]{zhang2017deconvolutional}
Yizhe Zhang, Dinghan Shen, Guoyin Wang, Zhe Gan, Ricardo Henao, and Lawrence
  Carin.
\newblock 2017.
\newblock Deconvolutional paragraph representation learning.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  4172--4182.

\bibitem[\protect\citename{Zhou \bgroup et al.\egroup }2013]{zhou2013improving}
Guangyou Zhou, Yang Liu, Fang Liu, Daojian Zeng, and Jun Zhao.
\newblock 2013.
\newblock Improving question retrieval in community question answering using
  world knowledge.
\newblock In {\em IJCAI}, volume~13, pages 2239--2245.

\end{thebibliography}

